RE-RecSys: An End-to-End system for recommending properties in Real-Estate domain

We propose an end-to-end real-estate recommendation system, RE-RecSys, which has been productionized in real-world industry setting. We categorize any user into 4 categories based on available historical data: i) cold-start users; ii) short-term users; iii) long-term users; and iv) short-long term users. For cold-start users, we propose a novel rule-based engine that is based on the popularity of locality and user preferences. For short-term users, we propose to use content-filtering model which recommends properties based on recent interactions of users. For long-term and short-long term users, we propose a novel combination of content and collaborative filtering based approach which can be easily productionized in the real-world scenario. Moreover, based on the conversion rate, we have designed a novel weighing scheme for different impressions done by users on the platform for the training of content and collaborative models. Finally, we show the efficiency of the proposed pipeline, RE-RecSys, on a real-world property and clickstream dataset collected from leading real-estate platform in India. We show that the proposed pipeline is deployable in real-world scenario with an average latency of <40 ms serving 1000 rpm.

==> Deployment.tex <==
\section{Deployment}


The deployment process for our recommendation system involves several key steps to ensure the accuracy and latency of
the API. The first step is to ingest user interaction data using a store and stream platform. This data is then pre-processed
and features are computed using a computation cluster, which enables us to quickly analyze and extract insights from
the data. Once the computed results are available at each level, they are pushed to Amazon RDS, which serves as our
central database for storing and retrieving the data. This enables us to efficiently manage and analyze large volumes of
data, and retrieve relevant information in real-time.

The next step in the deployment process involves the actual implementation of our recommendation engine. Whenever
a user on the platform hits the property display page, the recommendation engine is automatically invoked. The engine
fetches the user eligibility type and based on this type, invokes the relevant models and returns the response. The main
challenge in production is to keep the latency within 40ms, as any delay can have a significant impact on downstream
services across the platform.
To ensure this, we have designed our architecture with a focus on minimizing latency, and have implemented several
optimizations to ensure that our recommendation engine can provide accurate and timely responses to users. The entire
architecture of our recommendation system is depicted in the attached figure, which outlines the various components
and interactions involved in the data processing and recommendation generation.

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{deployment_diagram.png}
    \caption{Enter Caption}
    \label{fig:enter-label}
\end{figure}
